Accept Synthetic Objects as Real: End-to-End Training of Attentive Deep Visuomotor Policies for Manipulation in Clutter

Recent research demonstrated that it is feasible to end-to-end train multi-task deep visuomotor policies for robotic manipulation using variations of learning from demonstration (LfD) and reinforcement learning (RL). In this paper, we extend the capabilities of end-to-end LfD architectures to object manipulation in clutter. We start by introducing a data augmentation procedure called Accept Synthetic Objects as Real (ASOR). Using ASOR we develop two network architectures: implicit attention ASOR-IA and explicit attention ASOR-EA. Both architectures use the same training data (demonstrations in uncluttered environments) as previous approaches. Experimental results show that ASOR-IA and ASOR-EA succeed ina significant fraction of trials in cluttered environments where previous approaches never succeed. In addition, we find that both ASOR-IA and ASOR-EA outperform previous approaches even in uncluttered environments, with ASOR-EA performing better even in clutter compared to the previous best baseline in an uncluttered environment.

==> ExpTable.tex <==
\begin{table*}[ht]
\caption{Experimental results}
\vspace{0.1cm}
\label{tab:last_results}
\begin{tabular}{p{2cm}ccccccccccccc}
\cline{1-13}
\multicolumn{1}{|c|}{\multirow{3}{*}{{\textbf{\begin{tabular}[c]{@{}c@{}}\\Textual\\Command\\ Sentences\\ \\ \\ \end{tabular}}}}} & \multicolumn{7}{c|}{\multirow{2}{*}{{\textbf{Pick up ...}}}} & \multicolumn{5}{c|}{\multirow{2}{*}{{\textbf{Push ... from left to right}}}} &  \\
\multicolumn{1}{|c|}{} & \multicolumn{7}{c|}{} & \multicolumn{5}{c|}{} & \multicolumn{1}{c}{} \\ \cline{2-14}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}Red \\ Bowl\end{tabular}}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}White \\ Towel\end{tabular}}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}Blue \\ Ring\end{tabular}}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{  }c@{  }}Black \\Dumbbell \end{tabular}}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}White \\ Plate\end{tabular}}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}Red \\ Bubbles\end{tabular}}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}Mean \\ pick up\end{tabular}}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}Red \\ Bowl\end{tabular}}}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}White \\ Plate\end{tabular}}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}Blue \\ Box\end{tabular}}}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}B/W \\ QR-box\end{tabular}}}} & \multicolumn{1}{c}{\rotatebox[origin=c]{-90}{{\begin{tabular}[c]{@{}c@{}}Mean \\ Push\end{tabular}}}} & \multicolumn{1}{||c|}{\rotatebox[origin=c]{-90}{{
\begin{tabular}[c]{@{}c@{}}Mean\\\end{tabular}}}} \\ \hline
\\
\cline{1-1}
\multicolumn{1}{|c|}{\multirow{2}{*}{{\textbf{\begin{tabular}[c]{@{}c@{}}Method\end{tabular}}}}} & \multicolumn{12}{c}{\multirow{2}{*}{{\textbf{Benign Condition}}}} & \multicolumn{1}{c}{} \\
\multicolumn{1}{|c|}{} & \multicolumn{12}{c}{} & \multicolumn{1}{c}{} \\ \hline
\multicolumn{1}{|c|}{\textbf{(w/o TFA) (\%)}~\cite{rahmatizadeh2017vision}} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{40} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{43.3} & \multicolumn{1}{c|}{80} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{20} & \multicolumn{1}{c}{42.5} & \multicolumn{1}{||c|}{43.0} \\ \hline
\multicolumn{1}{|c|}{\textbf{with TFA (\%)}~\cite{Abolghasemi_2019_CVPR}} & \multicolumn{1}{c|}{80} & \multicolumn{1}{c|}{80} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{80} & \multicolumn{1}{c|}{\textbf{40}} & \multicolumn{1}{c|}{65.0} & \multicolumn{1}{c|}{\textbf{100}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c}{62.5} & \multicolumn{1}{||c|}{64.0} \\ \hline
\multicolumn{1}{|c|}{\textbf{Implicit Attention (\%)}} & \multicolumn{1}{c|}{80} & \multicolumn{1}{c|}{\textbf{100}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{40} & \multicolumn{1}{c|}{80} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{65.0} & \multicolumn{1}{c|}{80} & \multicolumn{1}{c|}{\textbf{70}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c}{67.5} & \multicolumn{1}{||c|}{66.0} \\ \hline
\multicolumn{1}{|c|}{\textbf{Explicit Attention (\%)}} & \multicolumn{1}{c|}{\textbf{90}} & \multicolumn{1}{c|}{\textbf{100}} & \multicolumn{1}{c|}{\textbf{80}} & \multicolumn{1}{c|}{\textbf{60}} & \multicolumn{1}{c|}{\textbf{100}} & \multicolumn{1}{c|}{\textbf{40}} & \multicolumn{1}{c|}{\textbf{78.3}} & \multicolumn{1}{c|}{\textbf{100}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{\textbf{90}} & \multicolumn{1}{c|}{\textbf{80}} & \multicolumn{1}{c}{\textbf{82.5}} & \multicolumn{1}{||c|}{\textbf{80.0}} \\ \hline
 & \multicolumn{12}{c}{\multirow{2}{*}{{\textbf{Cluttered Condition}}}} & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{12}{c}{} & \multicolumn{1}{c}{} \\ \hline
\multicolumn{1}{|c|}{\textbf{ Implicit Attention (\%)}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{40} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{\textbf{20}} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{80} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{40} & \multicolumn{1}{c}{57.5} & \multicolumn{1}{||c|}{53.0} \\ \hline
\multicolumn{1}{|c|}{\textbf{Explicit Attention (\%)}} & \multicolumn{1}{c|}{\textbf{80}} & \multicolumn{1}{c|}{\textbf{80}} & \multicolumn{1}{c|}{\textbf{80}} & \multicolumn{1}{c|}{\textbf{70}} & \multicolumn{1}{c|}{\textbf{90}} & \multicolumn{1}{c|}{\textbf{20}} & \multicolumn{1}{c|}{\textbf{70}} & \multicolumn{1}{c|}{\textbf{100}} & \multicolumn{1}{c|}{\textbf{70}} & \multicolumn{1}{c|}{\textbf{90}} & \multicolumn{1}{c|}{\textbf{70}} & \multicolumn{1}{c}{\textbf{82.5}} & \multicolumn{1}{||c|}{\textbf{75.0}} \\ \hline
\end{tabular}
\end{table*}



==> NotIncluded.tex <==



%The encoder, will receive the original image from the scene and returns a feature vector which will then be concatenated with the one-hot vectors representation of the object involved in the task. These vectors are extracted from the input sentence. The result will be fed to the generator. Generator's job is to reconstruct the original image plus an image masked with an attention map. Reconstructing both the raw image and masked image will help the network to retain all the relevant information including: robot's position, robot's position relative to the target object, gripper status, object position and etc. Since both encoder and generator have access to the one-hot vectors, encoder will be forced to include attention related information so that the generator be able to position the unmasked area based on both latent code and one-hot vectors. These images will then be fed to the discriminator. The Encoder($E$) and the Generator($G$) inner architecture used in this work are inspired by what had been proposed in~\cite{eslami2018neural}. The general VAE-GAN architecture is inspired by ~\cite{rahmatizadeh2017vision}. In this work we are investigating whether the attention helps the network to act robustly and recover from it's mistakes.



We used VAE-GAN to extract features from both raw images of the scene and masked images calculated by the TFA. Features extracted from raw images of the scene are needed to train the control network, however if we use the features extracted by the attention model, we are gonna miss lots of useful information which the controller network needs in order to perform, such as the robot position relative to the target object. Robot position can only be seen in the raw images, since the attention might not include the robot itself in the masked image we decided to extract features from both the raw and masked images. Figure~\ref{fig:adversarial_net} illustrates the network architecture we used to extract features from the raw and masked images.

% \subsection{Architecture overview}


\subsection{Formulation}
In this section, we will explain our formulation of the loss function and techniques we used in the training process.
 The Encoder will try to find a mapping between input data and the latent representation given the object's descriptors $z \sim E(x) = q(z|x,s,c)$. The generator will then reconstruct the input image $x$ using the learned distribution $x' \sim G(x) = P(x|z,s,c)$. 
 
 There is also the Discriminator network $D$, in the traditional GAN framework, the generator $G$ and the discriminator $D$ play an adversarial game. The generator objective is to generate realistic images and The discriminator is trying to classify the generated images as fake. The discriminator's objective to minimize is:
\begin{align*}
     - \EX_{x \sim P_{data}}[\log{D(x)}] - \EX_{z \sim P_{noise}}[\log{1-D(G(z))}]
\end{align*}
and the generator's objective is to minimize:
\begin{align*}
     -\EX_{z \sim P_{noise}}[\log{D(G(z))}]
\end{align*}
 
 Unlike the discriminators used in the traditional GAN, in this work the discriminator will be used as a classifier~\cite{salimans2016improved}. The classifier takes an image as input and tries to classify the image based on the object of interest's shape and color present in the image. The output of the discriminator is two one-hot vectors with the size of $n$ and $m$. These one-hot vectors are related to the object's shape and color respectively. To do semi-supervised learning, the data generated by the generator should also be used as input data to this classifier. We can simply change the output sizes to $n + 1$ and $m + 1$. When the discriminator wants to mark an image as fake it will classify it in the extra class that we added.
The network $D$ receives 3 types of images. $D$ receives raw from the dataset and masked images from our attention model and it should classify them into their corresponding class based on the object in them.
\begin{align*}
    \mathcal{L}_{real} =& - \EX_{x, s \sim p_{data}(x,s)} [\log{p_\mathit{model}(s|x,s < n + 1)}]\\
           & - \EX_{x, c \sim p_{data}(x,c)} [\log{p_{model}(c|x,c < m + 1)}]
\end{align*}


-------------- from the ASOR section


% We are going to compare two different architectures capable of performing in clutter. First architecture is similar to the one introduced in~\cite{rahmatizadeh2017vision} along with data-augmentation techniques. Second, we discuss an architecture which extracts attention and is better suited for cluttered environments. We used the publicly available dataset used in~\cite{Abolghasemi_2019_CVPR}. The dataset has single object demonstrations for two tasks: 1- Picking up something 2- Pushing Something. The dataset includes demonstrations with 8, 5 objects for picking up and pushing tasks respectively. Following our goal we won't record any additional demonstrations in clutter.

%Transforming single object demonstrations to demonstrations in clutter can be done synthetically by randomly placing objects cropped from other frames, somewhere in the scene. This way countless demonstrations can be generated with little effort.
% Figure~\ref{fig:data_aug} top section illustrates the augmentation process.

% https://docs.google.com/drawings/d/1wH--H5JU0afetFm3APVMyf3_QmvxKJh8AsBW2gs9fO8/edit?usp=sharing


% The synthetic objects may look natural to the human eye, however patterns on the cropped images can bias the network to easily detect the synthetic objects and remove them without learning what was intended. To address this, we recorded a small set of images without any object in them. These images only have the robot in random positions. We added two or three objects randomly to these empty images. Feeding these images containing only fake objects to the network and force it to remove all of them except the one present in the input sentence, prevents the described bias. Figure~\ref{fig:data_aug} bottom section illustrates this process. 

% https://docs.google.com/drawings/d/1EanaxvWvQD1AUZ7DyKmqFP1H4LcjqzbxRA99g8cysU8/edit?usp=sharing
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/data_augmentation2.pdf}
%     \caption{Top row images are empty images captured by randomly moving the robot. Middle row is the created by adding a random object to empty images. Bottom row is their the corresponding augmented image by randomly placing 1 or 2 additional objects.}
%     \label{fig:data_aug2}
%     %\vspace{-5mm}
% \end{figure}

% Now that we have pairs of corresponding images in which one image, only contains the object of interest and the other one contains all the other visual disturbances, we can train a network to receive the disturbed image as input and generate the image containing only the target object. On the other hand, this augmentation technique in theory can generate unlimited amount of training data for the network.




\subsection{Pairwise Feature Matching}
% Add equation
Training GANs is famous to be unstable. Feature matching is a way to improve the stability in training GANs~\cite{bao2017cvae}. Feature matching will force $G$ to generate images which match the statistics of the real data~\cite{salimans2016improved}. 


%\subsection{Semi-supervised learning}

% \subsection{Cycle Consistency}
% % Add equation
% The generator outputs an image with 6 channels. The first three channel are a reconstruction of the original image and the others are the masked image with attention. The reconstruction of original image reconstruction will then be used as input to the encoder. This input will then generate another set of masked and unmasked images after going through the encoder and the generator. We tried to reduce the cycle consistency by minimizing the difference between these two sets.
% \begin{align*}
%     x' &= G(E(x))\\
%     \mathcal{L}_{cyc} &= ||G(E(x'))) - x'||^2 
% \end{align*}
% where $x$ is the input image.

%\subsection{Training The Network}
The network illustrated in the figure~\ref{fig:adversarial_net} was trained end-to-end. Both the control and vision components were trained together. When such a large network is loaded to the GPUs due to the memory constraints the sequence size cannot be increased to a level that is required to properly train the controller. To overcome this limitation, after the end-to-end training is finished, we calculated the features for all the images in our dataset using the trained encoder and fine-tuned the controller using them with larger sequence size.


\subsection{Mixture Density Networks}
Our controller network is similar to what has been used in \cite{rahmatizadeh2017vision}. Features extracted by the encoder from the input images, will be used to train a 3 layer LSTM network As shown in figure~\ref{fig:adversarial_net}. The LSTM network receives the extracted feature from the input image in each timestamp and returns a 7-dimension vector corresponding to the next joints' angle. Instead of using mean squared error we used Mixture Density Network~\cite{bishop1994mixture} to calculate the LSTM loss. The controller network predicts a mixture of gaussians which tries to represent the next joint angle distribution. By sampling from such a mixture, we will have robot's next joint angle.

LSTM layers in our model have skip connections~\cite{graves2013generating}, meaning we concatenate the input to output of each and pass to the next layers and respectively we concatenate the outputs from all layers and pass through Fully Connected(FC) layers to predict the Gaussian kernel parameters $\mu_{i}$, $\sigma_{i}$. We also have another FC layer which outputs the mixing coefficient $\alpha_{i}(x)$. Since $\sum_{i=1}^{N}\alpha_{i}(x) = 1$ we used softmax activation for this layer. At last the controller network loss function defines as negative logarithmic likelihood~\cite{bishop1994mixture}:
\begin{align*}
    \mathcal{L}_{LSTM} = -ln{\sum_{i=1}^{n}\alpha_{i}(x)g_{i}(J_{t}|x)}
\end{align*}


In order to train our visual and controller networks, we selected two tasks. Pushing and picking up tasks are chosen and demonstrated for the network. 5 and 4 objects were chosen for demonstrating picking up and pushing task respectively. Figure~\ref{fig:objects} shows the objects used for demonstrations. We recorded the demonstrations using a PlayStation Eye camera with the frequency of 10 Hz. 150 demonstrations per object per task were recorded. we used the PlayStation controller to control the robot for all these demonstrations. All joint angles of the robot was recorded along with the corresponding images from the scene. Lynxmotion-AL5D doesn't have any feedback process, so we assumed whatever command we sent to the robot is executed successfully, We are essentially recording the commands we send to the robot and not the robot's current joint angles. As a results, the network is unable to detect any collision from the joint angles, it should try to detect collision from the input images.



To compare the performance of the a

To answer the second question, we compare our model to a similar work which is essentially our network without any TFA. In~\cite{rahmatizadeh2017vision} the network is trained on 5 tasks, however the tasks are limited compared to what we have here. In this work tasks can be performed on different objects whereas in the other work, tasks are bounded to the objects. This will make the tasks much harder because the robot's behaviours needs to be changed accordingly not only based on the task that it's performing but also based on the target object. Table ~\ref{tab:pick_up} and table ~\ref{tab:push} will compare these two networks' success rate in performing these tasks. We tested the networks for both of the tasks. We asked each network to perform the task 10 times for each distinct object.



The results show that there is a slight improvement in the success rate of performing these two tasks. However, the main difference between having TFA and not having it is that the model which uses TFA keeps trying even after failing to pick the object. To investigate this more statistically, we disturbed the robot physically during or after the robot grabs the object, disturbing the robot means we either forcefully got back the object from the robot or we slightly moved the object before the robot could completely grabs it. The model without attention never/rarely returned to pick the object, however the model with attention always retried to grab the object again after it was forcefully removed/moved-away from its gripper. The attention helps the model to better be aware of the target object's position. When the robot drops the object either by mistake or by external forces the attention locks on the object and the model goes back to pick the object again. Table~\ref{tab:recovery} will show the success rate of recovering from such a situation for the model using attention and without attention. 


\begin{table}
    \centering
    \setlength{\tabcolsep}{5pt}
    \caption{Success percentages over 10 trials for various tasks.}
    \label{tab:last_results}
    \begin{tabular}{|p{0.15cm}|p{1.7cm}|p{0.7cm}p{0.8cm}p{0.6cm}p{0.6cm}||p{0.6cm}p{0.6cm}|}
    \hline
    \multicolumn{2}{|c}{\multirow{2}{*}{Task spec.}} & \multicolumn{4}{|c||}{W/o clutter} & \multicolumn{2}{c|}{With clutter} \\
    \cline{3-8}
    % header - try to make these horizontal
    %\multicolumn{2}{|c|}{} & \rotatebox[origin=c]{-90}{w/o att.} & \rotatebox[origin=c]{-90}{with att.} & \rotatebox[origin=c]{-90}{ASOR IA} & \rotatebox[origin=c]{-90}{ASOR EA} & \rotatebox[origin=c]{-90}{ASOR IA} & \rotatebox[origin=c]{-90}{ASOR EA} \\
    % \cline{2-8}
    %\hline
    \multicolumn{2}{|c|}{} & {\scriptsize w/o att. \cite{rahmatizadeh2017vision}} & {\scriptsize with att. \cite{Abolghasemi_2019_CVPR}} & ASOR IA & ASOR EA & ASOR IA & ASOR EA \\
    % \cline{2-8}
    \hline    
    \multirow{7}{*}{\rotatebox[origin=c]{-90}{Pick up}} & Red Bowl & 70 & 80 & 80 & \bf{90} & 60 & \bf{80} \\
    & White Towel & 50 & 80 & \bf{100} & \bf{100} & 70 & \bf{100} \\
    & Blue Ring & 30 & 60 & 60 & \bf{80} & 40 & \bf{80} \\
    & {\scriptsize Black Dumbbell} & 40  & 50 & 40 & \bf{60} & 50 & \bf{70} \\
    & White Plate & 60 & 80 & 80 & \bf{100} & 60 & \bf{90} \\
    & {\scriptsize Red Bubblewrap} & 10 & \bf{40} & 30 & \bf{40} & \bf{20} & \bf{20} \\
    \cline{2-8}
    & \cellcolor{lightgray} Mean pick up &\cellcolor{lightgray} 43.3 & \cellcolor{lightgray}65.0 & \cellcolor{lightgray}65.0 &\cellcolor{lightgray} \bf{78.3} & \cellcolor{lightgray}50.0 & \cellcolor{lightgray}\bf{70.0} \\
    \hline
    \multirow{5}{*}{\rotatebox[origin=c]{-90}{Push to right}} & Red Bowl & 80 & \bf{100} & 80 & \bf{100} & 80 & \bf{100} \\
    & White Plate & 60 & 60 & \bf{70} & 60 & 50 & \bf{70} \\
    & Blue Box & 10 & 30 & 60 & \bf{90} & 50 & \bf{90} \\
    & BW QR-box & 20 & 60 & 60 & \bf{80} & 40 & \bf{70} \\
    & \cellcolor{lightgray} Mean push & \cellcolor{lightgray}42.5 & \cellcolor{lightgray}62.5 &\cellcolor{lightgray} 67.5 & \cellcolor{lightgray}\bf{82.5} &\cellcolor{lightgray} 57.5 & \cellcolor{lightgray}\bf{82.5} \\
    \hline
    \rowcolor{lightgray} \multicolumn{2}{c}{Overall mean} & 43.0 & 64.0 & 66.0 & 80.0 & 53.0 & 75.0 \\
    \hline
    \end{tabular}
    \vspace{-5mm}
\end{table}

Old abstract

Training end-to-end deep visuomotor policies for robotic arms performing range of tasks, including complex picking and placing, all trained on a single model has been accomplished before. Most of the proposed architectures are usually trained and tested in ideal setups without any distractor objects. A distractor object might be an object which the network never encountered during training such as a human hand or in more challenging cases it can be an object involved in other manipulation tasks. In this paper we propose data augmentation techniques along with a novel deep visuomotor architecture trained through demonstrations. The proposed architecture can successfully determine the target object among a wide range of distractor objects some of them involved in other manipulations, by utilizing the input sentence describing the task. We show that the proposed architecture can outperform variants of architectures in both benign and cluttered environments. We used a publicly available dataset containing single object demonstrations and no additional demonstrations is required in cluttered environment. 

Old intro


%Techniques used in computer vision is rapidly propagating into other fields. Robotics uses such techniques and architectures to extract information from the surrounding environment. However, robotic is not just about extracting better features or bounding boxes. Using the state of the art object detection, image segmentation and bounding box techniques doesn't translate to being able to grasp the detected object in the real world. Robotic challenges are not limited to approaching an object. Multi-task learning, multi-robot learning and performing the tasks in clutter are among the challenging aspects of robotics.

% https://docs.google.com/drawings/d/1bd3KBjWvS8fzPIZ5BEEFY4raOrwEnX7224UTBeGjws8/edit?usp=sharing
%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=\columnwidth]{Figures/overview.pdf}
%    \caption{The flow of commands for the end-to-end learning from demonstration model for robotic manipulation.}
%    \label{fig:overview}
%    \vspace{-7mm}
%\end{figure}

% There are multiple active approaches in robotics to address these challenges. Reinforcement Learning (RL) tries to address them by finding an optimal policy. The policy is learned during episodes of interacting with the environment and maximizing the reward earned in each interacting episode. Imitation Learning on the other hand is learning the optimal policy by looking at demonstrations made by an expert on how to act in different situations. In simple words, RL is like a child interacting with the environment to learn how to use his/her arm and imitation learning is like a child mimicking his/her parents.

% End to end training of deep visuomotor policies~\cite{rahmatizadeh2017vision} eliminates the need to use motion planning algorithms, learning how to grasp various types of objects and consequently reduces the complexity of training such policies. These policies can perform various tasks such as picking up, pushing, stacking, pouring and cleaning, all without separately learning how to do motion planning, grasping and robot control. In this work, we are going to describe an architecture which is trained using supervised data(demonstrations). Figure~\ref{fig:overview} is illustrating an overview of the general approach for Imitation Learning. First, a set of demonstrations for the tasks we expect the robot to learn needs to be recorded. Sequences of images from the robot's working area and commands sent to the robot by the demonstrator are among the information recorded during the demonstrations. The network's inputs includes but not limited to 1) a sentence describing the desired task 2) an image describing the state of the environment. The images contain information that might not be of any value for learning to perform the manipulation. The Visual Network's job is to condense the raw image into a vector(Primary Latent Encoding) orders of magnitude smaller. The motor network will then use the Primary Latent Encoding ($z$) to generate the next joint command for the robot to execute. Executing the latest command will change the state and a new observation describing it will be fed to the visual network and this cycle repeats until the desired task is performed.

% The motor network prediction is conditioned on the primary latent encoding. The primary latent encoding contains the important features extracted by the visual network. arm's and objects' poses are among these vital features. If the visual network is unaware of the desired task it will include the features corresponding to all the objects present in the scene. This will make the motor network's job difficult since it needs to find out the object of interest by itself. One possible brute force approach is to gather more demonstrations with variety of distractor objects in various poses so that the motor network training set includes most of the combinations. On the other hand, if the visual network learns to use the sentence describing the task, it can ignore the distractors and only include information related to the object of interest in $z$. In this work, we are going to discuss two different approaches to force the visual network to not include the irrelevant objects in the latent space.

%\textbf{Our Contributions:} The contributions of the paper are as follows:
%\textbf{1-} We describe a novel architecture for a visuomotor policy trained end-to-end from demonstrations. The proposed architecture relies on its attention module to extract segments of the image related to the task. The task is described to the network via a sentence. \textbf{2-} We show that the attention module allows the policy to perform in clutter as well. \textbf{3-} We show that, under both benign and cluttered environments the proposed architecture outperforms the model proposed in~\cite{rahmatizadeh2017vision, Abolghasemi_2019_CVPR}. \textbf{4-} The attention module can be trained end to end with the visual and control network and does not require additional training data or pixel level annotation of objects.




==> future_work.tex <==
\section{Future work}
\label{sec:Future}
In general, paying attention to more important parts of an image or video, results in faster reaction and less computation. Moreover, attention can really show its strength when it has been used in cluttered environments. It is not feasible and/or practical for a network to be able to perform the requested task in presence of arbitrary objects, which the network didn't see in the training samples. Attention can help the network ignore irrelevant parts of the environment and focus on what has been requested from it. One interesting future direction is to perform tasks in a cluttered environment without a significant drop in it's performance.
